nuSTORM - Neutrinos from STORed Muons: Proposal to the Fermilab PAC

The nuSTORM facility has been designed to deliver beams of electron neutrinos and muon neutrinos (and their anti-particles) from the decay of a stored muon beam with a central momentum of 3.8 GeV/c and a momentum acceptance of 10%. The facility is unique in that it will: 1. Allow searches for sterile neutrinos of exquisite sensitivity to be carried out; 2. Serve future long- and short-baseline neutrino-oscillation programs by providing definitive measurements of electron neutrino and muon neutrino scattering cross sections off nuclei with percent-level precision; and 3. Constitutes the crucial first step in the development of muon accelerators as a powerful new technique for particle physics. The document describes the facility in detail and demonstrates its physics capabilities. This document was submitted to the Fermilab Physics Advisory Committee in consideration for Stage I approval.

==> 0001_Title/Title.tex <==
%
\pagestyle{empty}
\thispagestyle{empty}
%
%========  Title page
%\begin{figure}[ht]
%  \centering{
%    \includegraphics[width=0.5\textwidth]{Logo_WB.png}}
%  \label{fig:Logo}
%\end{figure}
%
%\vspace{-5mm}
\title{Neutrinos from STORed Muons\\ Proposal\\ to the Fermilab Physics Advisory Committee}
%
\date{\today}
\clearpage

==> 001_Author_list/Author.tex <==
%
\author{D.~Adey}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{S.K.~Agarwalla}
\affiliation{Institute of Physics, Sachivalaya Marg, Sainik School Post, Bhubaneswar 751005, Orissa, India}
\author{C.M.~Ankenbrandt}\footnote{Also at Fermilab, P.O. Box 500, Batavia, IL 60510-5011, USA}
\affiliation{Muons Inc., 552 N. Batavia Avenue, Batavia, IL 60510, USA} 
\author{R.~Asfandiyarov}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{J.J.~Back}
\affiliation{Department of Physics, University of Warwick, Coventry, CV4 7AL, UK}
\author{G.~Barker}
\affiliation{Department of Physics, University of Warwick, Coventry, CV4 7AL, UK}
\author{E. Baussan}
\affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, F-67037 Strasbourg, France}
\author{R.~Bayes}
\affiliation{School of Physics and Astronomy, Kelvin Building, University of Glasgow, Glasgow G12 8QQ, Scotland, UK}
\author{S.~Bhadra}
\affiliation{Department of Physics and Astronomy, York University, 4700 Keele Street, Toronto, Ontario, M3J 1P3, Canada}
\author{V.~Blackmore}
\affiliation{Oxford University, Subdepartment of Particle Physics, Oxford, UK}
\author{A.~Blondel}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{S.A.~Bogacz}
\affiliation{Thomas Jefferson National Accelerator Facility, Newport News, VA, USA}
\author{C.~Booth}
\affiliation{University of Sheffield, Dept. of Physics and Astronomy, Hicks Bldg., Sheffield S3 7RH, UK}
\author{S.B.~Boyd}
\affiliation{Department of Physics, University of Warwick, Coventry, CV4 7AL, UK}
\author{A.~Bravar}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{S.J.~Brice}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{A.D.~Bross}\footnote{Corresponding author: bross@fnal.gov}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{F.~Cadoux}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{H.~Cease}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{A.~Cervera}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), Centro Mixto CSIC-UVEG, Edificio Institutos Investigaci\'on, Paterna, Apartado 22085, 46071 Valencia, Spain}
\author{J.~Cobb}
\affiliation{Oxford University, Subdepartment of Particle Physics, Oxford, UK}
\author{D.~Colling}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{P. Coloma}
\affiliation{Center for Neutrino Physics, Virginia Polytechnic Institute and State University. Blacksburg, VA 24061-0435}
\author{L.~Coney}
\affiliation{University of California, Riverside, CA, USA}
\author{A.~Dobbs}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{J.~Dobson}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{A.~Donini}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), Centro Mixto CSIC-UVEG, Edificio Institutos Investigaci\'on, Paterna, Apartado 22085, 46071 Valencia, Spain}
\author{P.~Dornan}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{M.~Dracos}
\affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, F-67037 Strasbourg, France}
\author{F.~Dufour}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{R.~Edgecock}
\affiliation{STFC Rutherford Appleton Laboratory, Chilton, Didcot, Oxfordshire, OX11 0QX, UK}
\author{J.~Evans}
\affiliation{School of Physics and Astronomy, The University of Manchester,  Oxford Road, Manchester, M13 9PL, UK}
\author{M.~Geelhoed}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{M.A.~George}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{T.~Ghosh}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), Centro Mixto CSIC-UVEG, Edificio Institutos Investigaci\'on, Paterna, Apartado 22085, 46071 Valencia, Spain}
\author{J.J.~G\'omez-Cadenas}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), Centro Mixto CSIC-UVEG, Edificio Institutos Investigaci\'on, Paterna, Apartado 22085, 46071 Valencia, Spain}
\author{A.~de~Gouv\^ea}
\affiliation{Northwestern University, Evanston, IL, USA}
\author{A.~Haesler} 
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{G.~Hanson}
\affiliation{University of California, Riverside, CA, USA}
\author{P.F.~Harrison}
\affiliation{Department of Physics, University of Warwick, Coventry, CV4 7AL, UK}
\author{M.~Hartz}\footnote{Also at Department of Physics, University of Toronto, 60 St. George Street, Toronto, Ontario, M5S 1A7, Canada}
\affiliation{Department of Physics and Astronomy, York University, 4700 Keele Street, Toronto, Ontario, M3J 1P3, Canada}
\author{P.~Hern\'andez}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), Centro Mixto CSIC-UVEG, Edificio Institutos Investigaci\'on, Paterna, Apartado 22085, 46071 Valencia, Spain}
\author{J.A.~Hernando~Morata}
\affiliation{Universidade de Santiago de Compostela (USC), Departamento de Fisica de Particulas, E-15706 Santiago de Compostela, Spain}
\author{P.~Hodgson}
\affiliation{University of Sheffield, Dept. of Physics and Astronomy, Hicks Bldg., Sheffield S3 7RH, UK}
\author{P.~Huber}
\affiliation{Center for Neutrino Physics, Virginia Polytechnic Institute and State University. Blacksburg, VA 24061-0435}
\author{A.~Izmaylov}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), Centro Mixto CSIC-UVEG, Edificio Institutos Investigaci\'on, Paterna, Apartado 22085, 46071 Valencia, Spain}
\author{Y.~Karadzhov}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{T.~Kobilarcik}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{J.~Kopp}
\affiliation{Max-Planck-Institut f\"{u}r Kernphysik, PO Box 103980, 69029 Heidelberg, Germany}
\author{L.~Kormos}
\affiliation{Physics Department, Lancaster University, Lancaster, LA1 4YB, UK}
\author{A.~Korzenev}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{Y.~Kuno}
\affiliation{Osaka University, Osaka, Japan}
\author{A.~Kurup}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{P.~Kyberd}
\affiliation{Brunel University, West London, Uxbridge, Middlesex UB8 3PH, UK}
\author{J.B.~Lagrange}
\affiliation{Kyoto University, Kyoto, Japan}
\author{A.~Laing}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), Centro Mixto CSIC-UVEG, Edificio Institutos Investigaci\'on, Paterna, Apartado 22085, 46071 Valencia, Spain}
\author{A.~Liu}\footnote{Also at Indiana University Bloomington, 107 S Indiana Ave, Bloomington, IN 47405, USA}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{J.M.~Link}
\affiliation{Center for Neutrino Physics, Virginia Polytechnic Institute and State University. Blacksburg, VA 24061-0435}
\author{K.~Long}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{K.~Mahn}
\affiliation{TRIUMF, 4004 Wesbrook Mall, Vancouver, B.C., V6T 2A3, Canada}
\author{C.~Mariani}
\affiliation{Center for Neutrino Physics, Virginia Polytechnic Institute and State University. Blacksburg, VA 24061-0435}
\author{C.~Martin}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{J.~Martin}
\affiliation{Department of Physics, University of Toronto, 60 St. George Street, Toronto, Ontario, M5S 1A7, Canada}
\author{N.~McCauley}
\affiliation{Department of Physics, Oliver Lodge Laboratory, University of Liverpool, Liverpool, L69 7ZE, UK}
\author{K.T.~McDonald}
\affiliation{Princeton University, Princeton, NJ, 08544, USA}
\author{O.~Mena}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), Centro Mixto CSIC-UVEG, Edificio Institutos Investigaci\'on, Paterna, Apartado 22085, 46071 Valencia, Spain}
\author{S.R.~Mishra}
\affiliation{Department of Physics and Astronomy, University of South Carolina, Columbia SC 29208, USA}
\author{N.~Mokhov}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{J.~Morfin}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{Y.~Mori}
\affiliation{Kyoto University, Kyoto, Japan}
\author{W.~Murray}
\affiliation{STFC Rutherford Appleton Laboratory, Chilton, Didcot, Oxfordshire, OX11 0QX, UK}
\author{D.~Neuffer}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{R.~Nichol}
\affiliation{Department of Physics and Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{E.~Noah}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{S.~Parke}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{M.A.~Palmer}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{S.~Pascoli}
\affiliation{Institute for Particle Physics Phenomenology,  Durham University, Durham, UK}
\author{J.~Pasternak}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{M.~Popovic}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{P.~Ratoff}
\affiliation{Physics Department, Lancaster University, Lancaster, LA1 4YB, UK}
\author{M.~Ravonel}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{M.~Rayner}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{S.~Ricciardi}
\affiliation{STFC Rutherford Appleton Laboratory, Chilton, Didcot, Oxfordshire, OX11 0QX, UK}
\author{C.~Rogers}
\affiliation{STFC Rutherford Appleton Laboratory, Chilton, Didcot, Oxfordshire, OX11 0QX, UK}
\author{P.~Rubinov}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{E.~Santos}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{A.~Sato}
\affiliation{Osaka University, Osaka, Japan}
\author{T.~Sen}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{E.~Scantamburlo}
\affiliation{University de Geneve, 24, Quai Ernest-Ansermet, 1211 Geneva 4, Switzerland}
\author{J.K.~Sedgbeer}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{D.R.~Smith}
\affiliation{Brunel University, West London, Uxbridge, Middlesex UB8 3PH, UK}
\author{P.J.~Smith}
\affiliation{University of Sheffield, Dept. of Physics and Astronomy, Hicks Bldg., Sheffield S3 7RH, UK}
\author{J.T.~Sobczyk}
\affiliation{Institute of Theoretical Physics, University of Wroclaw, pl. M. Borna 9,50-204, Wroclaw, Poland}
\author{L.~S$\o$by}
\affiliation{CERN,CH-1211, Geneva 23, Switzerland}
\author{F.J.P.~Soler}
\affiliation{School of Physics and Astronomy, Kelvin Building, University of Glasgow, Glasgow G12 8QQ, Scotland, UK}
\author{S.~Soldner-Rembold}
\affiliation{School of Physics and Astronomy, The University of Manchester,  Oxford Road, Manchester, M13 9PL, UK}
\author{M.~Sorel}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), Centro Mixto CSIC-UVEG, Edificio Institutos Investigaci\'on, Paterna, Apartado 22085, 46071 Valencia, Spain}
\author{P.~Snopok}\footnote{Also at Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\affiliation{Illinois Institute of Technology, Chicago, IL 60616}
\author{P.~Stamoulis}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), Centro Mixto CSIC-UVEG, Edificio Institutos Investigaci\'on, Paterna, Apartado 22085, 46071 Valencia, Spain}
\author{L.~Stanco}
\affiliation{INFN, Sezione di Padova, 35131 Padova, Italy}
\author{S.~Striganov}
\affiliation{Fermi National Accelerator Laboratory, Box 500, Batavia, IL 60510-5011, USA}
\author{H.A.~Tanaka}
\affiliation{Department of Physics and Astronomy, Hennings Building, The University of British Columbia, 6224 Agricultural Road, Vancouver, B.C., V6T 1Z1, Canada}
\author{I.J.~Taylor}
\affiliation{Department of Physics, University of Warwick, Coventry, CV4 7AL, UK}
\author{C.~Touramanis}
\affiliation{Department of Physics, Oliver Lodge Laboratory, University of Liverpool, Liverpool, L69 7ZE, UK}
\author{C.~D.~Tunnell}\footnote{Now at NikHEF, Amsterdam, The Netherlands}
\affiliation{Oxford University, Subdepartment of Particle Physics, Oxford, UK}
\author{Y.~Uchida}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{N.~Vassilopoulos}
\affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, F-67037 Strasbourg, France}
\author{M.O.~Wascko}
\affiliation{Physics Department, Blackett Laboratory, Imperial College London, Exhibition Road, London, SW7 2AZ, UK}
\author{A.~Weber}
\affiliation{Oxford University, Subdepartment of Particle Physics, Oxford, UK}
\author{M.J.~Wilking}
\affiliation{TRIUMF, 4004 Wesbrook Mall, Vancouver, B.C., V6T 2A3, Canada}
\author{E.~Wildner}
\affiliation{CERN,CH-1211, Geneva 23, Switzerland}
\author{W.~Winter}
\affiliation{Fakult\"at f\"ur Physik und Astronomie, Universit{\"a}t W{\"u}rzburg Am Hubland, 97074 W\"urzburg, Germany}
\author{U.K.~Yang}
\affiliation{School of Physics and Astronomy, The University of Manchester,  Oxford Road, Manchester, M13 9PL, UK}
\collaboration{The nuSTORM Collaboration}
%

==> 00_Executive_summary/def_temp.tex <==
%==============================================================================
%
% Temporary file: contains definitions for 01-Introduction:
% ---------------------------------------------------------
%
%=============================================================================


==> 01_Overview/def_temp.tex <==
%==============================================================================
%
% Temporary file: contains definitions for 01-Introduction:
% ---------------------------------------------------------
%
%=============================================================================


==> 03.5_Siting/def_temp.tex <==
%==============================================================================
%
% Temporary file: contains definitions for 01-Introduction:
% ---------------------------------------------------------
%
%=============================================================================


==> 03_Facility/def_temp.tex <==
%==============================================================================
%
% Temporary file: contains definitions for 01-Introduction:
% ---------------------------------------------------------
%
%=============================================================================


==> 04_FarDetector/def_temp.tex <==
%==============================================================================
%
% Temporary file: contains definitions for 01-Introduction:
% ---------------------------------------------------------
%
%=============================================================================


==> 05_NearDetector/def_temp.tex <==
%==============================================================================
%
% Temporary file: contains definitions for 01-Introduction:
% ---------------------------------------------------------
%
%=============================================================================


==> 06_Performance/def_temp.tex <==
%==============================================================================
%
% Temporary file: contains definitions for 01-Introduction:
% ---------------------------------------------------------
%
%=============================================================================


==> 07_OnC/def_temp.tex <==
%==============================================================================
%
% Temporary file: contains definitions for 01-Introduction:
% ---------------------------------------------------------
%
%=============================================================================


==> 99-Styles/GetPackages.tex <==
\usepackage{times}
\usepackage{bm}         % bold maths
\usepackage{amsmath,amssymb,bm,slashed} % need for subequations
\usepackage{amssymb}    % extra math symbols
\usepackage{graphicx}   % need for figures
\usepackage{verbatim}   % useful for program listings
\usepackage{color}      % use if color is used in text
\usepackage{subfigure}  % use for side-by-side figures
\usepackage{hyperref}   % use for hypertext links, including those to external documents and URLs
\usepackage{enumerate}

\usepackage{fmtcount}   % Allow counters to be printed with padding

\usepackage[square,comma,numbers,sort&compress]{natbib}



==> 99-Styles/nuSTORM-EoI-defs.tex <==
% Quantum mechanical notation
\newcommand{\bra}[1]{\ensuremath{\langle #1 |}}   % Bra vector
\newcommand{\ket}[1]{\ensuremath{| #1 \rangle}}   % Ket vector
\newcommand{\bigbra}[1]{\ensuremath{\big\langle #1 \big|}}   % Bra vector
\newcommand{\bigket}[1]{\ensuremath{\big| #1 \big\rangle}}   % Ket vector
\newcommand{\amp}[3]{\ensuremath{\left\langle #1 \,\left|\, #2%
                     \,\right|\, #3 \right\rangle}}  % QM amplitude
\newcommand{\sprod}[2]{\ensuremath{\left\langle #1 |%
                     #2 \right\rangle}}  % QM scalar product
\newcommand{\ev}[1]{\ensuremath{\left\langle #1 %
                     \right\rangle}} % Expectation value
\newcommand{\ds}[1]{\ensuremath{\! \frac{d^3#1}{(2\pi)^3 %
                     \sqrt{2 E_\vec{#1}}} \,}} % Spatial integral
\newcommand{\dst}[1]{\ensuremath{\! %
                     \frac{d^4#1}{(2\pi)^4} \,}} % Space-time integral
\newcommand{\tr}{\text{tr}}
\newcommand{\sgn}{\text{sgn}}
\newcommand{\diag}{\text{diag}}
\newcommand{\BR}{\text{BR}}

% Miscellaneous commands
\renewcommand{\vec}[1]{{\mathbf{#1}}}
\renewcommand{\Re}{{\text{Re}}}
\renewcommand{\Im}{{\text{Im}}}
\newcommand{\iso}[2]{{\ensuremath{{}^{#2}}\ensuremath{\rm #1}}}
\newcommand{\eps}{{\ensuremath{\epsilon}}}
\newcommand{\draftnote}[1]{{\bf\color{red} \MakeUppercase{#1}}}
\newcommand{\panm}[1]{{\color{blue} #1}}
\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\norm}[1]{\lVert#1\rVert}

\def\parenbar{\mathpalette\p@renb@r}
\def\p@renb@r#1#2{\vbox{%
  \ifx#1\scriptscriptstyle \dimen@.7em\dimen@ii.2em\else
  \ifx#1\scriptstyle \dimen@.8em\dimen@ii.25em\else
  \dimen@1em\dimen@ii.4em\fi\fi \offinterlineskip
  \ialign{\hfill##\hfill\cr
    \vbox{\hrule width\dimen@ii}\cr
    \noalign{\vskip-.3ex}%
    \hbox to\dimen@{$\mathchar300\hfil\mathchar301$}\cr
    \noalign{\vskip-.3ex}%
    $#1#2$\cr}}}

%
%.. Sanjib's commands:
\providecommand{\anmne}{\mbox{$\bar\nu_{\mu} \rightarrow \bar\nu_e$}} 
\providecommand{\nmne}{\mbox{$\nu_{\mu}\rightarrow\nu_e$}} 
\providecommand{\anm}{\mbox{$\bar\nu_\mu$}} 
\providecommand{\nm}{\mbox{$\nu_\mu$}}
\providecommand{\nue}{\mbox{$\nu_e$}} 
\providecommand{\ane}{\mbox{$\bar\nu_e$}} 
\providecommand{\enu}{\mbox{$E_\nu$}}
\providecommand{\piz}{\mbox{$\pi^0 $}}
\providecommand{\pip}{\mbox{$\pi^+$}} 
\providecommand{\pim}{\mbox{$\pi^-$}} 

